Dynamics of critical vortices on the torus and on the plane

We use the Bradlow parameter expansion to construct the metric tensor in the space of solutions of the Bogomolny equations for the Abelian Higgs model on a two-dimensional torus. Using this metric we study the dynamics and scattering of vortices on the torus within the geodesic approximation. For small torus volumes the metric is determined in terms of a small number of parameters. For large volumes the results provide a very precise approximation to the metric and dynamics on the plane.

==> results.tex <==
\subsection{Near the Bradlow limit}

Here we will examine the first few terms of the expansion in powers of 
$\epsilon$. These terms will describe quite accurately the structure 
of the metric for small values of $\epsilon$, or equivalently for
torus sizes which are not too large compared with the critical area of 
Bradlow. 

In Appendix~\ref{ap:order2} we give the first two non-zero orders of 
the expansion for arbitrary $q$. The first  term reduces in our case to the 
a constant curvature metric on the sphere of radius 
$\frac{\mathcal A}{\pi}$. The next term is given  by a
polynomial of forth degree in the variables $c_i/||c||$ and its
complex conjugate. By inspecting the form of the equations it is easy 
to realize that, in general, the elements of $||c||^2 g^{(n)}_{i j}$ are 
polynomials of degree $2n$ in $c_i/||c||$. Going over to the variable 
$Z$, we conclude that Nth order contribution to $\tilde f(Z,\overline Z)$
is a polynomial in $\frac{Z}{1 +|Z|^2}$ and its conjugate of degree 2n. 
Additional information about this polynomial follows from the
symmetries of the problem discussed earlier. To express the
restrictions  of these symmetries it is more convenient to go to the 
$(\theta,\varphi)$ coordinates defined in Eq.~\ref{eq:basistp}. 
{\bf meter aqui la discusion de las simetrias}


Finally, we conclude that the contribution to order $\epsilon^n$ 
to the function $\tilde f$, entering 
the expression~\ref{eq:basistpm} of the metric, has the form:
\begin{equation}
  \label{eq:expansi}
    \frac{\pi}{2}\tilde f^{(n)}(\theta,\varphi) = \sum_{jk}A^{(n)}_{jk} \cos^{2j}{\theta}
    \sin^{4k}{\theta} \cos^{2k}{2\varphi}
\end{equation}
The non-zero coefficients appearing  in this expression up to order 
 $\epsilon^5$ are collected in table~\ref{tab:metric}. The analytical
 expression of the second order coefficients are given in the appendix. 
 The rest have been extracted from our $40\times40$ grid of points up
 to machine double precision. 
 
\begin{table}
  \centering
  \begin{tabular}{|c|c||c|c|}
    \hline
    & $\mathbf{O(3)}$ & & $\mathbf{O(2)}$ \\
    \hline
    $A^{(3)}_{00}$ & $1.57\ 24\ 57\ 43\ 63\ 76\ 56(1)\times 10^{-1}$ &
    $A^{(2)}_{00}$ & $2.09\ 85\ 65\ 63\ 87\ 72\ 34\ 78\ 07\times 10^{-1}$ \\
    \hline
    $A^{(3)}_{10}$ & $-7.35\ 97\ 58\ 95\ 32\ 71\ 25\times 10^{-1} $ & 
    $A^{(2)}_{10}$ & $-6.29\ 56\ 96\ 91\ 63\ 17\ 04 39\ 78\times 10^{-1}$ \\
    \hline
    $A^{(3)}_{20}$ & $4.40\ 39\ 77\ 74\ 02\ 36\ 00\times 10^{-1}$ & 
    & $\mathbf{O(5)}$ \\
    \hline
    & $\mathbf{O(4)}$ & $A^{(5)}_{00}$ & $3.24\ 86\ 80\ 02\ 33\ 12\ 76\times
    10^{-1}$ \\
    \hline
    $A^{(4)}_{00}$ & $2.56\ 44\ 31\ 24\ 38\ 37\ 31\ 64(1)\times 10^{-1}$&
    $A^{(5)}_{10}$ & $-1.59\ 28\ 19\ 34\ 17\ 36\ 19\ 6$\\
    \hline
    $A^{(4)}_{10}$ & $-1.09\ 63\ 43\ 50\ 68\ 01\ 26(2)$&
    $A^{(5)}_{20}$ & $2.35\ 30\ 76\ 79\ 79\ 16\ 14\ 0$\\
    \hline
    $A^{(4)}_{20}$ & $1.12\ 62\ 17\ 59\ 37\ 90\ 85(1)$&
    $A^{(5)}_{30}$ & $-1.33\ 17\ 87\ 41\ 82\ 85\ 50\ 3$\\
    \hline
    $A^{(4)}_{30}$ & $-3.23\ 47\ 12\ 72\ 58\ 54\ 03(4)\times 10^{-1}$&
    $A^{(5)}_{40}$ & $2.44\ 37\ 72\ 51\ 19\ 98\ 28\times 10^{-1}$\\
    \hline
    $A^{(4)}_{01}$ & $-2.62\ 60\ 73\ 46\ 53\ 83\ 54(1)\times 10^{-1}$&
    $A^{(5)}_{01}$ & $-4.46\ 53\ 65\ 89\ 63\ 78\ 00\times 10^{-1}$\\
    \hline
     & &
    $A^{(5)}_{11}$ & $4.62\ 92\ 29\ 53\ 30\ 50\ 51\times 10^{-1}$\\
    \hline
  \end{tabular}
  \caption{Coefficients of the expansion of the metric up to fifth order.}
  \label{tab:metric}
\end{table}

An important check of our results follows from the computation of the
volume of fiber. As mentioned previously the result obtained from the
leading term already match with the volume calculated in 
Refs.~\cite{Shah:1994us,Manton:1998kq}. Hence,  the $n > 1$
contribution to the  volume must vanish. This leads to the conditions:
\begin{equation}
\sum_{ j k } A_{jk}^{(n)}  \frac{\Gamma\left( j+\frac{1}{2} \right)
\left[(2k)!\right]^2}
{(k!)^22^{2k+1}\Gamma\left(j+2k+\frac{3}{2}\right)}=0 
\end{equation}
which are nicely satisfied by our coefficients up to machine double
precision.  

We will now analyze the two-vortex dynamics that follows from our 
fifth order metric. This is governed by the Hamiltonian
\begin{equation}
  H = \frac{1}{4\tilde f(\theta,\varphi)}\left(
    p_\theta^2 + \frac{p_\varphi^2}{\sin^2\theta}
  \right)
\end{equation}
The equations of motion are
\begin{subequations}
  \begin{equation}
    \dot\theta = \frac{p_\theta}{2\tilde f}
  \end{equation}
  \begin{equation}
    \dot\varphi = \frac{p_\varphi}{2\tilde f\sin^2\theta}
  \end{equation}
  \begin{equation}
    \dot p_\theta = \frac{1}{2\tilde f}\left(
      2E\frac{\partial\tilde f}{\partial\theta} +
      p_\varphi^2\frac{\cos\theta}{\sin^3\theta} 
    \right)
  \end{equation}
  \begin{equation}
    \dot p_\varphi = \frac{E}{\tilde f}\frac{\partial\tilde
      f}{\partial\varphi} 
  \end{equation}
\end{subequations}
Where $E$ is the energy of the system, that is conserved. These 
equations can be easily integrated numerically to obtain the
trajectories in vortex moduli space.  

Notice, that up to third order, the metric is independent of 
$\varphi$. Hence, $p_\varphi$ is 
a conserved quantity, and the problem is  integrable. 
In this case, the equation for the trajectory in the moduli
space is given by
\begin{equation}
  \varphi_f = \varphi_0 +
  \int_{\theta_0}^{\theta_f}\frac{d\theta}{\sin^2{\theta}
    \sqrt{\frac{\tilde f(\theta)}{b^2} - \frac{1}{\sin^2{\theta}}}}
\end{equation}
where $b=\frac{\sqrt{E}}{2p_\varphi}$. 

 
An interesting mathematical question is whether the two vortex 
dynamics on the torus is integrable for all values of $\epsilon$. 
As we have seen, this is the case up to third order in the expansion.
In the next subsection we will mention that it is also the case in the
$\epsilon \longrightarrow 1$ limit, since then we recover rotational 
invariance and angular momentum becomes a conserved quantity. Our metric
calculations could be used to give a numerical and/or  analytical answer 
to this question. We will not attempt to study that point here. Instead 
we will address the much simpler problem of obtaining and describing 
the Poincare maps obtained from the third order and fifth  order
metric. Results are displayed in Fig.~\ref{fig:poincare} for two values 
of $\epsilon$. We see signs of how some  invariant-tori  seem to be
destroyed, pointing to the non-integrability of the metric truncated 
to fifth order. This is not surprising and does not conflict with the 
conjectured integrability for all values of $\epsilon$. Our results 
nonetheless can be considered  as a first step, which might help in 
finding that at the relevant region of phase space where to look. 




\begin{figure}[htbp]
  \centering
  \mbox{
    \subfigure[Poicare map for $\epsilon=0.4$ and $E=15.0$ for the first 3
    orders.]{\includegraphics[width=7.55cm]{fig/Poincare_eps=040_O=3}}
    \subfigure[Poicare map for $\epsilon=0.4$ and $E=15.0$ for the first 5
    orders.]{\includegraphics[width=7.55cm]{fig/Poincare_eps=040_O=5}}
  }
  \mbox {
    \subfigure[Detail of the Poicare map for $\epsilon=0.4$ and
    $E=50.0$ for the first 3
    orders.]{\includegraphics[width=7.55cm]{fig/PoincareDet_eps=040_O=3}} 
    \subfigure[Detail of the Poicare map for $\epsilon=0.4$ and
    $E=50.0$ for the first 5
    orders.]{\includegraphics[width=7.55cm]{fig/PoincareDet_eps=040_O=5}} 
  }
  \caption{Examples of Poicare maps for the dynamics near the Bradlow limit.}
  \label{fig:poincare}
\end{figure}




\subsection{Dynamics of vortices in the plane ($\epsilon\rightarrow 1$
  limit)}

The dynamics of the Abelian Higgs model in $\mathbb R^2$ is a well
studied problem, both analytically~\cite{Samols:1990kd,Samols:1991ne}
and numerically~\cite{Samols:1991ne}. We know~\cite{Samols:1990kd}
that we can write the metric as
\begin{equation}
  ds^2 = F^2(|u|)\ dud\overline{u}
\end{equation}
Once the function $F(|u|)$ is obtained, the dynamics in the geodesic
approximation is completely determined. The form of the function
$F(|u|)$  has been deduced analytically for the special case of
asymptotically separated vortices~\cite{Manton:2002wb}, and has also
been studied numerically several
times\cite{Samols:1990kd,Samols:1991ne}. In this paper   we will 
use our expansion method  to obtain a precise determination 
of $F(|u|)$ for all values of $|u|$.

We will naturally assume that, if the torus is large enough
compared both with the typical size  of  vortices, and with the
distance between them, the \emph{dynamics} will be accurately described 
by the one in $\mathbb R^2$. This means that, at least formally,
we can calculate the desired function $F(|u|)$ as
\begin{equation}
  \label{eq:Ae}
  F^2(|u|) = \lim_{\epsilon\rightarrow 1}A(\epsilon)\sum_{n=1}^\infty
  g^{(n)}(u,\overline u)\epsilon^n
\end{equation}
We have allowed for a normalization constant $A(\epsilon)$ that does 
not affect the dynamics of vortices.

From Eq.~\ref{eq:metu} we can see that the function
$g^{(n)}(u,\overline u)$ is the product  of $\tilde f$ and a
known function  arising from the change of variables. We will first 
study the behaviour of the latter  factors in the limit $\epsilon
\longrightarrow 1$. The factor contains known functions of  the 
complex variable $w$, which is proportional to $u/l_1$. 
The linear extent of the torus $l_1$ and $l_2$ are proportional to
$1/(1-\epsilon)$, so that taking the $\epsilon\longrightarrow 1$ limit
at fixed $u$ and aspect ratio $\tau$ amounts to taking $w
\longrightarrow 0$. Hence, this factor becomes
\begin{equation}
  \left( \frac{2\pi q}{l} \right)^2
  |\vartheta_4(0)|^4\frac{|\vartheta_1(w)|^2
    |\vartheta_4(w)|^2}{\left( |\vartheta_2(w)|^2
      + |\vartheta_3(w)|^2 \right)^2}
  \stackrel{w\rightarrow 0}{\longrightarrow} 
  \frac{4\pi^2Z_2^2}{(1+Z_0^2)^2}(1-\epsilon)^2|u|^2
\end{equation}
where\footnote{For the rectangular symmetric case $l_1=l_2$, the
  numerical values of $Z_0$ and $Z_2$ are
  \begin{eqnarray*}
    Z_0 & = & -1-\sqrt{2} \\
    Z_2 & = & -1.18\ 91\ 73\ 93\ 79\ 71\ 08\ 15
  \end{eqnarray*}
} $Z_2=-\frac{1}{2}\frac{\vartheta_3(0)\vartheta_4^4(0)}
{\vartheta_2(0)}$, and $Z_0 = -\vartheta_3(0)/\vartheta_2(0)$. 

In analysing the $\epsilon\rightarrow 1$ limit of the metric, we will find it 
useful to write $\epsilon=e^{-\delta}$ and replace  the limit by $\delta
\longrightarrow 0$. Our assumption about the behaviour of the metric
for large volumes now becomes 
\begin{equation}
  \label{eq:Ae}
  F^2(|u|) = \lim_{\delta \rightarrow o}{\tilde A}(\delta) \delta^2
  \frac{4\pi^2Z_2^2}{(1+Z_0^2)^2}|u|^2 \sum_{n=1}^\infty
  {\tilde f}^{(n)}(u\sqrt{\pi q \delta},\overline u \sqrt{\pi q
    \delta}) e^{-n \delta} 
\end{equation}
It is clear that as $\delta$ tends to zero, more terms in the series
become relevant. It is tempting to assume that the infinite sum tends        
to an integral over the variable $y=n\delta$. This would imply the
following behaviour of the coefficients:
\begin{equation}
  \label{eq:CoeBeh}
  \lim_{n \longrightarrow  \infty} {\tilde
    f}^{(n)}\left(u\sqrt{\frac{\pi qy}{n}},\overline u \sqrt{\frac{\pi
        qy}{n}}\right) n^\alpha = h(|u|\sqrt{y})  
\end{equation}
In this case the limiting function $h(|u|\sqrt{y})$ would be related 
to $F^2(|u|)$ as follows:
\begin{equation}
  \label{eq:metricplane}
    F^2(|u|) =
      \frac{4\pi^2Z_2^2}{(1+Z_0^2)^2}|u|^2 \int_{0}^\infty
        e^{-y} h(|u|\sqrt{y})\, dy
	\end{equation}
which is essentially a Laplace transform. 	

With our results for ${\tilde f}^{(n)}$ up to  $n=40$ and a set of
values of $u$ spanning a $40\times 40$ grid we have analysed the 
validity of Eq.~\ref{eq:CoeBeh}. For that purpose we have plotted in
Fig.~\ref{fig:funch} the coefficients of $n\ge 35$ and all values 
of $u$ in the range. The smoothness and thinness of the resulting 
curve, approximating $h(x)$, is a test of our scaling hypothesis. 
Errors, signalled by  the spread of the values, grow with $x$. 
For example, including all coefficients $n>20$  gives essentially the 
same curve with many more points up to $x\approx 5$, but with 
considerable more spread (but similarly small values) for larger $x$. 


\EPSFIGURE[h]{fig/coeff.eps}{\label{fig:funch} We plot the left-hand
side of Eq.~\ref{eq:CoeBeh} for $n$ in the range 35-40, and fixed
$x=|u|\sqrt{y}$.}

The  function $h(x)$ for small $x$, as determined from 
our results,  fits nicely to a behaviour of the form
\begin{equation}
  \label{eq:w0}
    h(x) = a - bx^4 + O(x^5)
    \end{equation}
    where $a=0.335(1)$ and $b=0.0102(6)$.
This expansion implies that for small values of the argument 
the metric function $F^2(|u|)$ behaves as:
\begin{equation}
  \label{eq:r0}
  F^2(|u|) =
  \frac{4\pi^2Z_2^2}{(1+Z_0^2)^2}
  \left( a|u|^2 - 2b|u|^6 \right) + O(|u|^7)
\end{equation}
	
To compute the points of Fig.~\ref{fig:funcf}, we will use our
computation of $40$ orders and a similar scaling argument. We can
obtain the value of the metric in one point $|u_f|$ by using different
points of our grid and different values of $\epsilon$. If $\epsilon$
is large enough, the effects of the replicas is negligible, and we
should obtain the same value for the metric using these different
values of $\epsilon$ and different points of the grid. The differences
gives us a measure of the effect of the replicas and of the
truncation, that can be used as an estimation of the error. In
Fig.~\ref{fig:funcf} we can see (in red points) the metric computed
with this argument, our expansion  for short distances
(Eq.~\ref{eq:r0}), and the asymptotic expansion of
Ref.~\cite{Manton:2002wb} given by  
\begin{equation}
  \label{eq:metricas}
  F^2(|u|) \stackrel{|u|\rightarrow \infty}{\longrightarrow} 
  1-8\sqrt{2}K_0(4|u|)
\end{equation}
where $K_0(x)$ is the modified Bessel function of the second kind.

\EPSFIGURE[h]{fig/deffunc.eps}{\label{fig:funcf}The metric computed
  using 40 orders of the Bradlow parameter expansion (red points),
  versus the $|u|\rightarrow 0$ approximation Eq.~\ref{eq:r0} (green
  dashed line) and the asymptotic form of the metric
  Eq.~\ref{eq:metricas} (black solid line).} 


\subsubsection{Scattering of vortices on the plane}

Once the function $F(|u|)$ has been obtained, it is trivial to compute
the dynamics of the vortices. The Lagrangian, when written in polar
coordinates $u = re^{\imath\theta}$, is given by:
\begin{equation}
  T = F^2(r)\left[\dot r^2 + r^2\dot\theta^2\right]
\end{equation}
Since the energy is conserved, and we have rotational invariance
($p_\theta$ is also conserved), the system is integrable, and we have 
\begin{equation}
  \theta_f = \pi - \int^\infty_{r_f}
  \frac{dr}{r\sqrt{\frac{r^2}{b^2}F^2(r) - 1}} 
\end{equation}
where $b^2=\frac{p_\theta^2}{4T}$ is the \emph{impact parameter}. In
particular, if we call $r_m$ the minimum distance between one vortex
and the centre of mass during the trajectory, the scattering angle is
given by 
\begin{equation}
  \theta_{sc} = \pi - 2\int_{r_m}^{\infty}
  \frac{dr}{r\sqrt{\frac{r^2}{b^2}F^2(r) - 1}} 
\end{equation}

Using our numerical data of
Fig.~\ref{fig:funcf} we can calculate these integrals. For values of
$r > 5$ we will use the asymptotic form of the metric, and for 
$r<0.5$ we can use our approximation Eq.~(\ref{eq:r0}). For the
intermediate values we will use the cubic spline interpolating
polynomial. In the Fig.~\ref{fig:scatt} we have some examples of
trajectories for different values of the impact parameter.  

\EPSFIGURE[h]{fig/scatt.eps}{\label{fig:scatt}Scattering trajectories
  of two vortices.} 

We can also plot the scattering angle versus the impact parameter. The
results are shown in Fig.~\ref{fig:angle}. The errors here are
computed in the following way: We compute the spline interpolation
polynomial for the points in which we know the value of $F^2(|u|)$,
that with the asymptotic behaviour, and 
the small $r$ approximation gives us the complete function $F^2(r)$,
and then a scattering angle for each impact parameter. Then we change
the spline interpolation polynomial by changing the position of the
points according to it's error, and we obtain a different
scattering angle. The differences between the different scattering
angles measures how the errors in the function $F^2(|u|)$ propagates
to the scattering angle. We have repeated this procedure 1000 times,
and using this value, we have an estimation of the value and the error
of the scattering angle.

\EPSFIGURE[h]{fig/angle.eps}{\label{fig:angle}Scattering Angle
  vs. impact parameter.} 

% Local Variables: 
% mode: latex
% TeX-master: "paper"
% End: 

